Robust Model Predictive Control for Linear Systems with State and Input Dependent Uncertainties

This paper presents a computationally efficient robust model predictive control law for discrete linear time invariant systems subject to additive disturbances that may depend on the state and/or input norms. Despite the dependency being non-convex, we are able to capture it exactly for input dependency and approximately for state dependency in at most a second order cone programming problem. The formulation has linear complexity in the planning horizon length. The approach is thus amenable to efficient real-time implementation with a guarantee on recursive feasibility and global optimality. Robust position control of a satellite is considered as an illustrative example.

==> future.tex <==
\section{Future Work}
\label{sec:future}

This section outlines some future questions and possible extensions to the RMPC
law (\ref{eq:mpc_problem}). One possible line of work is to extend the noise
model (\ref{eq:uncertainty_set}) to handle input and state vector
\textit{direction} dependence. Indeed, to reduce conservatism some applications
involve direction-dependent noise such as the full version of the Gates model
\cite{Gates1963}. Some applications also define a non-convex $\mathcal U$, for
example
$\mathcal U=\{0\}\cup(\mathcal U_{\text{i}}\setminus\mathcal U_{\text{o}})$
where $\mathcal U_{\text{i}}\subset\mathcal U_{\text{o}}$ are two convex sets
such that $\mathcal U_{\text{i}}$ defines the set of non-zero input values that
the actuators cannot reproduce. This occurs due to e.g. RCS thruster
impulse-bit. While the state constraint (\ref{eq:rpi_v3}) can handle this
situation, Theorem~\ref{thm:recursive_feasibility} does not apply for a
non-convex $\mathcal U$ since its proof requires convexity. Furthermore,
(\ref{eq:input_constraint}) becomes a non-convex constraint. This problem was
previously handled in continuous time via lossless convexification
\cite{Acikmese2007,Acikmese2011,Blackmore2012} and mixed integer programming
\cite{Schouwenaars2006}, however no proof of recursive feasibility has yet been
proposed for uncertain discrete time systems. Last but not least, the
computation of $\mathcal I$ via \cite{Kvasnica2015} is expensive and sometimes
ineffective for the high-dimensional systems dealt with here. Moreover, it
requires over-approximating noise as independent, over-approximating ellipsoids
as polytopes and carries the assumption that $N=1$. Recent work on controllable
set computation for convex optimal control problems has the potential to speed
up and remove this conservatism \cite{Dueri2016}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "root"
%%% End:

